Algorithmic Building Blocks for Asymmetric Memories

The future of main memory appears to lie in the direction of new non-volatile memory technologies that provide strong capacity-to-performance ratios, but have write operations that are much more expensive than reads in terms of energy, bandwidth, and latency. This asymmetry can have a significant effect on algorithm design, and in many cases it is possible to reduce writes at the cost of reads. In this paper, we study which algorithmic techniques are useful in designing practical write-efficient algorithms. We focus on several fundamental algorithmic building blocks including unordered set/map implemented using hash tables, ordered set/map implemented using various binary search trees, comparison sort, and graph traversal algorithms including breadth-first search and Dijkstra's algorithm. We introduce new algorithms and implementations that can reduce writes, and analyze the performance experimentally using a software simulator. Finally we summarize interesting lessons and directions in designing write-efficient algorithms.

==> BFS-table-io.tex <==
\begin{table*}[!ht]
\centering
\small
\def\arraystretch{1.1}
\setlength{\tabcolsep}{6.5pt}
\small
    \begin{tabular}{l|rrr|rrr||rrr|rrr}
    \toprule
    \multicolumn{13}{c}{$\wcost{}=10$} \\
    \hline
    \textbf{Algorithm} & \multicolumn{3}{c|}{\textbf{Classic BFS}} & \multicolumn{3}{c||}{\textbf{BFS based on RA}} & \multicolumn{3}{c|}{\textbf{Classic Bidir.\ BFS}} & \multicolumn{3}{c}{\textbf{Bidir.\ BFS based on RA}} \\
    \hline
    \textbf{Cache Size} & \multicolumn{1}{c}{\textbf{500}} & \multicolumn{1}{c}{\textbf{2000}} & \multicolumn{1}{c|}{\textbf{10000}} & \multicolumn{1}{c}{\textbf{500}} & \multicolumn{1}{c}{\textbf{2000}} & \multicolumn{1}{c||}{\textbf{10000}} & \multicolumn{1}{c}{\textbf{500}} & \multicolumn{1}{c}{\textbf{2000}} & \multicolumn{1}{c|}{\textbf{10000}} & \multicolumn{1}{c}{\textbf{500}} & \multicolumn{1}{c}{\textbf{2000}} & \multicolumn{1}{c}{\textbf{10000}} \\
    \hline
    \textbf{2D Grid} & 80.18 & 77.72 & 56.74 & 17.13 & 8.15  & 6.25  & 67.80 & 67.04 & 55.53 & 13.14 & 6.27  & 4.76 \\
    \textbf{3D Grid} & \textit{73.85} & 69.49 & 58.60 & 130.86 & 51.16 & 10.18 & \textit{42.44} & 41.16 & 39.29 & 57.98 & 15.65 & 3.82 \\
    \textbf{PA Roadmap} & \textit{36.50} & 33.42 & 12.89 & 59.10 & 11.84 & 1.44  & \textit{39.76} & 38.46 & 19.39 & 53.24 & 8.52  & 1.24 \\
    \textbf{TX Roadmap} & \textit{28.42} & 25.14 & 10.44 & 46.36 & 9.36  & 1.18  & 28.27 & 26.95 & 12.37 & 22.89 & 4.37  & 0.69 \\
    \textbf{Stan Webgraph} & \textit{79.41} & \textit{64.64} & \textit{24.39} & 291.99 & 198.08 & 56.18 & 18.48 & 17.93 & 15.62 & 15.75 & 7.71  & 1.93 \\
    \textbf{NDU Webgraph} & \textit{13.84} & \textit{12.70} & \textit{10.20} & 132.71 & 98.04 & 35.58 & 7.80  & 7.73  & 7.54  & 6.90  & 3.90  & 0.75 \\
    \textbf{DBLP network} & \textit{77.19} & \textit{66.16} & \textit{23.67} & 213.43 & 166.84 & 69.63 & 11.53 & 11.22 & 9.91  & 3.84  & 1.61  & 0.56 \\
    \textbf{Youtube network} & \textit{37.92} & \textit{32.59} & \textit{24.06} & 159.43 & 135.92 & 90.72 & 7.58  & 7.50  & 7.38  & 1.17  & 0.51  & 0.17 \\
    \midrule
        \multicolumn{13}{c}{$\wcost{}=100$} \\
    \hline
    \textbf{Algorithm} & \multicolumn{3}{c|}{\textbf{Classic BFS}} & \multicolumn{3}{c||}{\textbf{BFS based on RA}} & \multicolumn{3}{c|}{\textbf{Classic Bidir.\ BFS}} & \multicolumn{3}{c}{\textbf{Bidir.\ BFS based on RA}} \\
    \hline
    \textbf{Cache Size} & \multicolumn{1}{c}{\textbf{500}} & \multicolumn{1}{c}{\textbf{2000}} & \multicolumn{1}{c|}{\textbf{10000}} & \multicolumn{1}{c}{\textbf{500}} & \multicolumn{1}{c}{\textbf{2000}} & \multicolumn{1}{c||}{\textbf{10000}} & \multicolumn{1}{c}{\textbf{500}} & \multicolumn{1}{c}{\textbf{2000}} & \multicolumn{1}{c|}{\textbf{10000}} & \multicolumn{1}{c}{\textbf{500}} & \multicolumn{1}{c}{\textbf{2000}} & \multicolumn{1}{c}{\textbf{10000}} \\
    \hline
    \textbf{2D Grid} & 635.55 & 618.76 & 469.43 & 92.57 & 22.78 & 6.72  & 514.72 & 511.85 & 470.75 & 62.97 & 18.27 & 5.35 \\
    \textbf{3D Grid} & 564.06 & 547.11 & 464.38 & 514.41 & 232.35 & 44.27 & 319.44 & 316.96 & 307.65 & 235.59 & 77.39 & 12.06 \\
    \textbf{PA Roadmap} & \textit{286.43} & 261.57 & 107.03 & 324.45 & 70.03 & 3.01  & 326.74 & 316.39 & 163.60 & 289.47 & 47.04 & 2.87 \\
    \textbf{TX Roadmap} & \textit{223.08} & 197.38 & 86.83 & 252.58 & 54.70 & 2.79  & 234.83 & 224.27 & 107.59 & 128.80 & 22.98 & 1.51 \\
    \textbf{Stan Webgraph} & \textit{436.30} & \textit{402.38} & 157.17 & 831.09 & 624.48 & 245.12 & 142.48 & 141.21 & 131.58 & 91.63 & 50.12 & 13.65 \\
    \textbf{NDU Webgraph} & \textit{107.13} & \textit{99.79} & 79.27 & 565.07 & 450.23 & 190.85 & 70.85 & 70.32 & 68.82 & 45.32 & 28.97 & 6.04 \\
    \textbf{DBLP network} & \textit{594.58} & \textit{522.66} & 175.08 & 874.18 & 731.33 & 357.35 & 102.67 & 100.58 & 89.70 & 26.40 & 12.78 & 4.54 \\
    \textbf{Youtube network} & \textit{260.17} & \textit{239.10} & 189.98 & 769.01 & 711.41 & 547.67 & 69.10 & 68.57 & 67.61 & 9.44  & 4.37  & 1.47 \\
    \bottomrule
\end{tabular}
\caption{\label{tbl:bfs-iocost}
I/O costs of BFS implementations on different cache sizes.  Numbers of r/w transfers are from Table~\ref{tbl:bfs-raw}.  Italic-font number indicates that the classic implementation has a lower I/O cost in that setting.
}
\end{table*}



==> BFS-table-rw.tex <==
\begin{table*}[!ht]
\centering
\small
\def\arraystretch{1.1}
    \begin{tabular}{l|rrrrrr|rrrrrr}
    \toprule
    \multicolumn{1}{c|}{\textbf{Algorithm}} & \multicolumn{6}{c|}{\textbf{Classic BFS}}      & \multicolumn{6}{c}{\textbf{BFS based on RA}} \\
    \cline{1-13}
    \multicolumn{1}{c|}{\textbf{Cache Size}} & \multicolumn{2}{c}{\textbf{500}} & \multicolumn{2}{c}{\textbf{2000}} & \multicolumn{2}{c|}{\textbf{10000}} & \multicolumn{2}{c}{\textbf{500}} & \multicolumn{2}{c}{\textbf{2000}} & \multicolumn{2}{c}{\textbf{10000}} \\
    \cline{1-13}
    \textbf{} & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c}{\textbf{WT}} & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c}{\textbf{WT}} & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c|}{\textbf{WT}} & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c}{\textbf{WT}} & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c}{\textbf{WT}} & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c}{\textbf{WT}} \\
    \hline

    \textbf{2D Grid} & 18.47 & 6.17  & 17.60 & 6.01  & 10.88 & 4.59  & 8.75  & 0.84  & 6.52  & 0.16  & 6.20  & 0.01 \\
    \textbf{3D Grid} & 19.38 & 5.45  & 16.42 & 5.31  & 13.51 & 4.51  & 88.24 & 4.26  & 31.03 & 2.01  & 6.39  & 0.38 \\
    \textbf{PA Roadmap} & 8.73  & 2.78  & 8.07  & 2.54  & 2.43  & 1.05  & 29.61 & 2.95  & 5.37  & 0.65  & 1.26  & 0.02 \\
    \textbf{TX Roadmap} & 6.79  & 2.16  & 6.01  & 1.91  & 1.95  & 0.85  & 23.45 & 2.29  & 4.32  & 0.50  & 1.00  & 0.02 \\
    \textbf{Stan Webgraph} & 39.75 & 3.97  & 27.11 & 3.75  & 9.63  & 1.48  & 232.09 & 5.99  & 150.70 & 4.74  & 35.19 & 2.10 \\
    \textbf{NDU Webgraph} & 3.47  & 1.04  & 3.02  & 0.97  & 2.52  & 0.77  & 84.67 & 4.80  & 58.91 & 3.91  & 18.33 & 1.73 \\
    \textbf{DBLP Network} & 19.70 & 5.75  & 15.43 & 5.07  & 6.85  & 1.68  & 140.01 & 7.34  & 104.12 & 6.27  & 37.67 & 3.20 \\
    \textbf{Youtube Network} & 13.23 & 2.47  & 9.64  & 2.29  & 5.63  & 1.84  & 91.70 & 6.77  & 71.98 & 6.39  & 39.95 & 5.08 \\

    \midrule
    \multicolumn{1}{c|}{\textbf{Algorithm}} & \multicolumn{6}{c|}{\textbf{Classic Bidirectional BFS}}      & \multicolumn{6}{c}{\textbf{Bidirectional BFS based on RA}} \\
    \cline{1-13}
    \multicolumn{1}{c|}{\textbf{Cache Size}} & \multicolumn{2}{c}{\textbf{500}} & \multicolumn{2}{c}{\textbf{2000}} & \multicolumn{2}{c|}{\textbf{10000}} & \multicolumn{2}{c}{\textbf{500}} & \multicolumn{2}{c}{\textbf{2000}} & \multicolumn{2}{c}{\textbf{10000}} \\
    \cline{1-13}
    \textbf{} & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c}{\textbf{WT}} & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c}{\textbf{WT}} & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c|}{\textbf{WT}} & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c}{\textbf{WT}} & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c}{\textbf{WT}} & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c}{\textbf{WT}} \\
    \hline

    \textbf{2D Grid} & 18.14 & 4.97  & 17.61 & 4.94  & 9.39  & 4.61  & 7.60  & 0.55  & 4.94  & 0.13  & 4.69  & 0.01 \\
    \textbf{3D Grid} & 11.66 & 3.08  & 10.52 & 3.06  & 9.47  & 2.98  & 38.24 & 1.97  & 8.80  & 0.69  & 2.90  & 0.09 \\
    \textbf{PA Roadmap} & 7.87  & 3.19  & 7.58  & 3.09  & 3.37  & 1.60  & 27.00 & 2.62  & 4.25  & 0.43  & 1.06  & 0.02 \\
    \textbf{TX Roadmap} & 5.31  & 2.30  & 5.03  & 2.19  & 1.79  & 1.06  & 11.12 & 1.18  & 2.30  & 0.21  & 0.60  & 0.01 \\
    \textbf{Stan Webgraph} & 4.70  & 1.38  & 4.24  & 1.37  & 2.74  & 1.29  & 7.32  & 0.84  & 3.00  & 0.47  & 0.63  & 0.13 \\
    \textbf{NDU Webgraph} & 0.80  & 0.70  & 0.77  & 0.70  & 0.74  & 0.68  & 2.63  & 0.43  & 1.12  & 0.28  & 0.16  & 0.06 \\
    \textbf{DBLP network} & 1.40  & 1.01  & 1.29  & 0.99  & 1.05  & 0.89  & 1.33  & 0.25  & 0.37  & 0.12  & 0.12  & 0.04 \\
    \textbf{Youtube network} & 0.74  & 0.68  & 0.71  & 0.68  & 0.69  & 0.67  & 0.25  & 0.09  & 0.08  & 0.04  & 0.02  & 0.01 \\

    \bottomrule
\end{tabular}
\caption{\label{tbl:bfs-raw}
Numbers of read and write transfers of four BFS implementations on different cache sizes.  Numbers are r/w transfers per vertex per \textbf{10} queries.  We pick the number 10 to fit the numbers in one table.  Cache size is measured by the number of 64-bytes cache-lines.}
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\end{table*}



==> BFS-table-stat-sigmod.tex <==
\begin{table}[!ht]
\centering
\small
\def\arraystretch{1.1}
    \begin{tabular}{l|rr|rr}
    \toprule
          & \multicolumn{2}{c|}{\textbf{Unidirectional search}} & \multicolumn{2}{c}{\textbf{Bidirectional search}} \\
    \cline{2-5}
          & \multicolumn{1}{p{.8cm}<{\centering}}{\textbf{depth}} & \multicolumn{1}{p{1.2cm}<{\centering}|}{\textbf{average frontier size}} & \multicolumn{1}{p{1.2cm}<{\centering}}{\textbf{depth}}  & \multicolumn{1}{p{1.2cm}<{\centering}}{\textbf{average frontier size}} \\
    \hline
    \textbf{2D Grid} & 1571.4 & 636.4 & 370.2 & 1102.8 \\
    \textbf{3D Grid} & 229.9 & 4349.7 & 49.3  & 4628.9 \\
    \textbf{PA Roadmap} & 574.5 & 1893.1 & 163.9 & 2718.3 \\
    \textbf{TX Roadmap} & 748.6 & 1804.9 & 174.7 & 2102.1 \\
    \textbf{Stan Webgraph} & 107.1 & 2383.4 & 3.5   & 3782.8 \\
    \textbf{NDU Webgraph} & 29.2  & 11155.1 & 3.8   & 2053.5 \\
    \textbf{DBLP Network} & 16.1  & 19694.4 & 3.9   & 1420.1 \\
    \textbf{Youtube Network} & 15.8 & 71828.5 & 2.7 & 107.4 \\
    \bottomrule
    \end{tabular}%
  \caption{The depths (number of levels in the shortest-path tree) and frontier sizes (number of vertices) during the search processes.  Note that the numbers are averaged from multiple searches.}
  \label{tab:BFS-stats}%
\end{table}%


==> dijk-fig.tex <==
\begin{figure*}
\begin{center}
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{../figs/dijk/dijk10-planar} \centering{\small (a) $\wcost=10$, sparse graphs}
    \end{minipage}
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{../figs/dijk/dijk10-social} \centering{\small (b) $\wcost=10$, social networks}
    \end{minipage}
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{../figs/dijk/dijk100-planar} \centering{\small (c) $\wcost=100$, sparse graphs}
    \end{minipage}
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{../figs/dijk/dijk100-social} \centering{\small (d) $\wcost=100$, social networks}
    \end{minipage}
\vspace{-.5em}
    \captionof{figure}{\label{fig:dijk} The trends of the I/O costs of classic Dijkstra (grey) and phased Dijkstra (red) on different graphs with varied cache sizes.
    Graphs used in the experiment are shown in Section~\ref{sec:graph} and categorized into sparse (almost planar) graphs and social networks.
    Each number of the I/O cost is geometric mean of the four graphs in that category (the exact numbers are given in Table~\ref{tbl:dijk-weighted}).
    Phased Dijkstra performs consistently better in all cases except when both the cache size and the asymmetry $\wcost{}$ are small.
    }
\end{center}
\end{figure*} 

==> dijk-other-table.tex <==
\begin{table}[htbp]
  \centering
  \small
  \def\arraystretch{1.1}
    \begin{tabular}{@{ }l@{ }|r@{ }r@{ }@{ }r@{ }r@{ }@{ }r@{ }r@{ }@{ }r@{ }r@{ }}
    \toprule
   \multicolumn{1}{@{}c@{ }|}{\textbf{Priority Queue Size}}       & \multicolumn{2}{c}{\textbf{30\%}} & \multicolumn{2}{c}{\textbf{40\%}} & \multicolumn{2}{c}{\textbf{50\%}} & \multicolumn{2}{c}{\textbf{60\%}} \\
\cline{1-9}          & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c}{\textbf{WT}} & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c}{\textbf{WT}} & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c}{\textbf{WT}} & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c}{\textbf{WT}} \\
    \hline
    \textbf{2D Grid} & 8.4   & 1.10  & 8.6   & 1.11  & 8.9   & 1.11  & 9.3   & 1.11 \\
    \textbf{3D Grid} & 33.7  & 1.12  & 28.9  & 1.12  & 25.6  & 1.12  & 23.3  & 1.12 \\
    \textbf{PA Roadmap} & 2.7   & 0.48  & 2.8   & 0.52  & 3.0   & 0.58  & 3.2   & 0.66 \\
    \textbf{TX Roadmap} & 2.6   & 0.48  & 2.7   & 0.53  & 2.9   & 0.59  & 3.1   & 0.66 \\
    \textbf{Stan Webgraph} & 94.4  & 1.02  & 82.9  & 1.02  & 72.1  & 1.02  & 67.1  & 1.02 \\
    \textbf{NDU Webgraph} & 26.1  & 1.01  & 22.8  & 1.01  & 20.2  & 1.03  & 18.5  & 1.04 \\
    \textbf{DBLP Network} & 75.1  & 1.10  & 64.9  & 1.10  & 57.3  & 1.10  & 51.5  & 1.11 \\
    \textbf{Youtube Network} & 183.8 & 1.11  & 161.5 & 1.11  & 144.4 & 1.12  & 134.9 & 1.12 \\
    \bottomrule
    \end{tabular}%
  \caption{Number of read and write transfers of phased Dijkstra on different priority queue's size.  The overall percentage of priority queue and vertex map varies from 30\% to 60\% comparing to the cache size, which is 10,000 cache-lines.}
  \label{tab:dijk-perc}%
\end{table}%


==> dijk-table-io.tex <==
\begin{figure*}[!ht]
\centering
\small
\def\arraystretch{1.1}
    \begin{tabular}{l|r@{ }@{ }@{ }r@{ }@{ }@{ }r|r@{ }@{ }@{ }r@{ }@{ }@{ }r||r@{ }@{ }@{ }r@{ }@{ }@{ }r|r@{ }@{ }@{ }r@{ }@{ }@{ }r} \toprule
          & \multicolumn{6}{c||}{$\bm{\wcost{}=10}$}             & \multicolumn{6}{c}{$\bm{\wcost{}=100}$} \\
\cline{2-13}
    & \multicolumn{3}{c|}{\textbf{Classic}} & \multicolumn{3}{c||}{\textbf{Phased Dijkstra}} & \multicolumn{3}{c|}{\textbf{Classic}} & \multicolumn{3}{c}{\textbf{Phased Dijkstra}} \\
%\cline{2-13}
\hline
    \multicolumn{1}{c|}{\textbf{Cache Size}} & \multicolumn{1}{c}{\textbf{2k}} & \multicolumn{1}{c}{\textbf{10k}} & \multicolumn{1}{c|}{\textbf{50k}} & \multicolumn{1}{c}{\textbf{2k}} & \multicolumn{1}{c}{\textbf{10k}} & \multicolumn{1}{c||}{\textbf{50k}} & \multicolumn{1}{c}{\textbf{2k}} & \multicolumn{1}{c}{\textbf{10k}} & \multicolumn{1}{c|}{\textbf{50k}} & \multicolumn{1}{c}{\textbf{2k}} & \multicolumn{1}{c}{\textbf{10k}} & \multicolumn{1}{c}{\textbf{50k}} \\
    \hline
    \textbf{2D Grid} & 59.12 & 28.03 & 22.40 & 17.16 & 14.70 & 13.15 & 497.81 & 238.87 & 192.21 & 118.26 & 114.34 & 106.83 \\
    \textbf{3D Grid} & 171.17 & 102.82 & 41.73 & 137.80 & 39.36 & 16.62 & 1478.93 & 871.17 & 343.56 & 238.97 & 140.13 & 113.13 \\
    \textbf{PA Roadmap} & 49.18 & 10.25 & 5.13  & 40.26 & 7.09  & 3.80  & 421.41 & 83.10 & 41.19 & 128.98 & 53.90 & 28.67 \\
    \textbf{TX Roadmap} & 48.68 & 10.38 & 5.08  & 47.58 & 7.15  & 3.74  & 417.56 & 84.35 & 40.96 & 134.49 & 54.59 & 28.36 \\
    \textbf{Stan Webgraph} & {\textit{218.61}} & 147.28 & 49.72 & 414.92 & 91.20 & 22.64 & 1850.27 & 1232.24 & 401.84 & 507.73 & 182.81 & 101.93 \\
    \textbf{NDU Webgraph} & 178.41 & 97.26 & 21.65 & 110.87 & 32.70 & 12.52 & 1559.37 & 836.30 & 169.74 & 209.91 & 123.90 & 72.87 \\
    \textbf{DBLP Network} & {\textit{228.70}} & 153.37 & 55.91 & 352.28 & 75.75 & 20.97 & 1997.66 & 1325.22 & 468.37 & 453.08 & 174.67 & 105.87 \\
    \textbf{Youtube Network} & {\textit{263.78}} & 192.06 & 150.14 & 847.91 & 172.50 & 43.60 & 2321.03 & 1679.39 & 1310.77 & 949.28 & 272.78 & 138.32 \\
    \bottomrule
    \end{tabular}%
\captionof{table}{\label{tbl:dijk-weighted}
The I/O costs on different Dijkstra implementations on different cache size.  The write-read ratio $\wcost{}$ are selected to be typical projected values 10 (latency, bandwidth) and 100 (energy).  Results are based on the numbers in Table~\ref{tbl:dijk-raw}.}
\end{figure*}


==> dijk-table-rw.tex <==
\begin{figure*}[!ht]
\centering
\small
\def\arraystretch{1.1}
    \begin{tabular}{l|rr|rr|rr|rr@{ }@{ }r|rr@{ }@{ }r|rr@{ }@{ }r} \toprule
          & \multicolumn{6}{c|}{\textbf{Classic Dijkstra using binary heap}} & \multicolumn{9}{c}{\textbf{Phased Dijkstra}} \\
\cline{1-16}
    \multicolumn{1}{c|}{\textbf{Cache Size}} & \multicolumn{2}{c|}{\textbf{2k}} & \multicolumn{2}{c}{\textbf{10k}} & \multicolumn{2}{c|}{\textbf{50k}} & \multicolumn{3}{c|}{\textbf{2k}} & \multicolumn{3}{c|}{\textbf{10k}} & \multicolumn{3}{c}{\textbf{50k}} \\
%\cline{1-16}\cline{1-16}
\hline
    \textbf{Graph Instance} & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c|}{\textbf{WT}} & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c|}{\textbf{WT}} & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c|}{\textbf{WT}} & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c}{\textbf{WT}} &  & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c}{\textbf{WT}} & & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c}{\textbf{WT}} \\
    \hline
    \textbf{2D Grid} & 10.37 & 4.87  & 4.61  & 2.34  & 3.53  & 1.89  & 5.93  & 1.12  & (1)   & 3.62  & 1.11  & (1)   & 2.74  & 1.04  & (1) \\
    \textbf{3D Grid} & 25.87 & 14.53 & 17.44 & 8.54  & 8.20  & 3.35  & 126.56 & 1.12  & (383) & 28.16 & 1.12  & (44)  & 5.90  & 1.07  & (1) \\
    \textbf{PA Roadmap} & 7.82  & 4.14  & 2.16  & 0.81  & 1.12  & 0.40  & 30.40 & 0.99  & (202) & 1.89  & 0.52  & (1)   & 1.04  & 0.28  & (1) \\
    \textbf{TX Roadmap} & 7.69  & 4.10  & 2.16  & 0.82  & 1.09  & 0.40  & 37.93 & 0.97  & (262) & 1.88  & 0.53  & (1)   & 1.01  & 0.27  & (1) \\
    \textbf{Stan Webgraph} & 37.31 & 18.13 & 26.73 & 12.06 & 10.60 & 3.91  & 404.61 & 1.03  & (100) & 81.02 & 1.02  & (16)  & 13.83 & 0.88  & (2) \\
    \textbf{NDU Webgraph} & 24.97 & 15.34 & 15.14 & 8.21  & 5.19  & 1.65  & 99.86 & 1.10  & (132) & 22.57 & 1.01  & (24)  & 5.81  & 0.67  & (3) \\
    \textbf{DBLP Network} & 32.14 & 19.66 & 23.17 & 13.02 & 10.08 & 4.58  & 341.08 & 1.12  & (131) & 64.75 & 1.10  & (24)  & 11.53 & 0.94  & (4) \\
    \textbf{Youtube Network} & 35.19 & 22.86 & 26.80 & 16.53 & 21.18 & 12.90 & 836.64 & 1.13  & (477) & 161.36 & 1.11  & (93)  & 33.08 & 1.05  & (18) \\
    \bottomrule
    \end{tabular}%
\captionof{table}{\label{tbl:dijk-raw}
Number of read and write transfers of different Dijkstra implementations on different cache size.  Numbers are normalized to read or write transfers per vertex.  We ran SSSP queries on 10 different randomly-chosen source nodes.  Numbers in the parentheses are the average phases.}
\end{figure*}


==> dijk-table.tex <==
\begin{figure*}[!ht]
\centering
\footnotesize
\def\arraystretch{1.2}
    \begin{tabular}{l|rr|rr|rr|rr@{ }@{ }r|rr@{ }@{ }r|rr@{ }@{ }r} \toprule
          & \multicolumn{6}{c|}{\textbf{Classic Dijkstra using binary heap}} & \multicolumn{9}{c}{\textbf{Phased Dijkstra}} \\
\cline{1-16}
    \multicolumn{1}{c|}{\textbf{Cache Size}} & \multicolumn{2}{c|}{\textbf{2k}} & \multicolumn{2}{c}{\textbf{10k}} & \multicolumn{2}{c|}{\textbf{50k}} & \multicolumn{3}{c|}{\textbf{2k}} & \multicolumn{3}{c|}{\textbf{10k}} & \multicolumn{3}{c}{\textbf{50k}} \\
%\cline{1-16}\cline{1-16}
\hline
    \textbf{Graph Instance} & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c|}{\textbf{WT}} & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c|}{\textbf{WT}} & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c|}{\textbf{WT}} & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c}{\textbf{WT}} &  & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c}{\textbf{WT}} & & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c}{\textbf{WT}} \\
    \hline
    \textbf{2D Grid} & 10.37 & 4.87  & 4.61  & 2.34  & 3.53  & 1.89  & 5.93  & 1.12  & (1)   & 3.62  & 1.11  & (1)   & 2.74  & 1.04  & (1) \\
    \textbf{3D Grid} & 25.87 & 14.53 & 17.44 & 8.54  & 8.20  & 3.35  & 126.56 & 1.12  & (383) & 28.16 & 1.12  & (44)  & 5.90  & 1.07  & (1) \\
    \textbf{PA Roadmap} & 7.82  & 4.14  & 2.16  & 0.81  & 1.12  & 0.40  & 30.40 & 0.99  & (202) & 1.89  & 0.52  & (1)   & 1.04  & 0.28  & (1) \\
    \textbf{TX Roadmap} & 7.69  & 4.10  & 2.16  & 0.82  & 1.09  & 0.40  & 37.93 & 0.97  & (262) & 1.88  & 0.53  & (1)   & 1.01  & 0.27  & (1) \\
    \textbf{Stan Webgraph} & 37.31 & 18.13 & 26.73 & 12.06 & 10.60 & 3.91  & 404.61 & 1.03  & (100) & 81.02 & 1.02  & (16)  & 13.83 & 0.88  & (2) \\
    \textbf{NDU Webgraph} & 24.97 & 15.34 & 15.14 & 8.21  & 5.19  & 1.65  & 99.86 & 1.10  & (132) & 22.57 & 1.01  & (24)  & 5.81  & 0.67  & (3) \\
    \textbf{DBLP Network} & 32.14 & 19.66 & 23.17 & 13.02 & 10.08 & 4.58  & 341.08 & 1.12  & (131) & 64.75 & 1.10  & (24)  & 11.53 & 0.94  & (4) \\
    \textbf{Youtube Network} & 35.19 & 22.86 & 26.80 & 16.53 & 21.18 & 12.90 & 836.64 & 1.13  & (477) & 161.36 & 1.11  & (93)  & 33.08 & 1.05  & (18) \\
    \bottomrule
    \end{tabular}%
\captionof{table}{\label{tbl:dijk-raw}
Number of read and write transfers of different Dijkstra implementations on different cache sizes.  Numbers are normalized to read or write transfers per vertex.  We ran SSSP queries on 10 different randomly-chosen source nodes.  Numbers in the parentheses are the average phases.}
    \begin{tabular}{l|r@{ }@{ }@{ }r@{ }@{ }@{ }r|r@{ }@{ }@{ }r@{ }@{ }@{ }r||r@{ }@{ }@{ }r@{ }@{ }@{ }r|r@{ }@{ }@{ }r@{ }@{ }@{ }r} \toprule
          & \multicolumn{6}{c||}{$\bm{\wcost{}=10}$}             & \multicolumn{6}{c}{$\bm{\wcost{}=100}$} \\
\cline{2-13}
    & \multicolumn{3}{c|}{\textbf{Classic}} & \multicolumn{3}{c||}{\textbf{Phased Dijkstra}} & \multicolumn{3}{c|}{\textbf{Classic}} & \multicolumn{3}{c}{\textbf{Phased Dijkstra}} \\
%\cline{2-13}
\hline
    \multicolumn{1}{c|}{\textbf{Cache Size}} & \multicolumn{1}{c}{\textbf{2k}} & \multicolumn{1}{c}{\textbf{10k}} & \multicolumn{1}{c|}{\textbf{50k}} & \multicolumn{1}{c}{\textbf{2k}} & \multicolumn{1}{c}{\textbf{10k}} & \multicolumn{1}{c||}{\textbf{50k}} & \multicolumn{1}{c}{\textbf{2k}} & \multicolumn{1}{c}{\textbf{10k}} & \multicolumn{1}{c|}{\textbf{50k}} & \multicolumn{1}{c}{\textbf{2k}} & \multicolumn{1}{c}{\textbf{10k}} & \multicolumn{1}{c}{\textbf{50k}} \\
    \hline
    \textbf{2D Grid} & 59.12 & 28.03 & 22.40 & 17.16 & 14.70 & 13.15 & 497.81 & 238.87 & 192.21 & 118.26 & 114.34 & 106.83 \\
    \textbf{3D Grid} & 171.17 & 102.82 & 41.73 & 137.80 & 39.36 & 16.62 & 1478.93 & 871.17 & 343.56 & 238.97 & 140.13 & 113.13 \\
    \textbf{PA Roadmap} & 49.18 & 10.25 & 5.13  & 40.26 & 7.09  & 3.80  & 421.41 & 83.10 & 41.19 & 128.98 & 53.90 & 28.67 \\
    \textbf{TX Roadmap} & 48.68 & 10.38 & 5.08  & 47.58 & 7.15  & 3.74  & 417.56 & 84.35 & 40.96 & 134.49 & 54.59 & 28.36 \\
    \textbf{Stan Webgraph} & {\textit{218.61}} & 147.28 & 49.72 & 414.92 & 91.20 & 22.64 & 1850.27 & 1232.24 & 401.84 & 507.73 & 182.81 & 101.93 \\
    \textbf{NDU Webgraph} & 178.41 & 97.26 & 21.65 & 110.87 & 32.70 & 12.52 & 1559.37 & 836.30 & 169.74 & 209.91 & 123.90 & 72.87 \\
    \textbf{DBLP Network} & {\textit{228.70}} & 153.37 & 55.91 & 352.28 & 75.75 & 20.97 & 1997.66 & 1325.22 & 468.37 & 453.08 & 174.67 & 105.87 \\
    \textbf{Youtube Network} & {\textit{263.78}} & 192.06 & 150.14 & 847.91 & 172.50 & 43.60 & 2321.03 & 1679.39 & 1310.77 & 949.28 & 272.78 & 138.32 \\
    \bottomrule
    \end{tabular}%
\captionof{table}{\label{tbl:dijk-weighted}
The I/O costs on different Dijkstra implementations on different cache sizes.  The write-read ratio $\wcost{}$ are selected to be typical projected values 10 (latency, bandwidth) and 100 (energy).  Results are based on the numbers in Table~\ref{tbl:dijk-raw}.}
\end{figure*}


==> graph-abs.tex <==
\section{Graph Traversal Algorithms}

In this paper, we discuss two of the most commonly-used graph-traversing algorithms: Breadth-first search (BFS), and Dijkstra's Algorithm.
Our goal is to show that with appropriate implementations, these algorithms can write much fewer to the main memory, comparing to the classic ones.
Due to the page limit, here we abstract our approaches and conclusions, and provide the full version in Appendix~\ref{sec:graph-traversal}.

\input{BFS-fig}

\subsection{Breadth-First Search}

We discussed our implementations and experiment results on breadth-first searches (BFS) on undirected graph traversing or searching.
Our algorithms compute the single-source shortest paths (SSSP) or pairwise shortest-paths (given the specific source and target) on unweighted graphs, which can further apply to graph radii estimation, eccentricity estimation and betweenness centrality, and as a basic building block for other graph algorithms like graph connectivity, reachability, bridges, biconnected components, and strongly connected components.

\mysubparagraph{Implementations.}
The classic implementation of BFS keeps a queue with size $n$, and an array of boolean flags with size $n$ indicating that each vertex is visited or not during the search.
This implementation requires at most 2 writes for each vertex, and the overall I/O cost of BFS $Q(n,m)=O(\wcost{}n+m)$~\cite{blelloch2016efficient}.
This bound is asymptotic optimal for arbitrary graphs since the output of BFS has size $O(n)$.
However, a number applications (e.g., s-t shortest-path or connectivity, graph radii estimation or eccentricity estimation) have output size $O(1)$, which allow techniques utilizing the \smallmem{} and reducing the number of writes.

The key observation to improve the write-efficiency is that, at any time, we only need the information of three consecutive frontiers.
We hence use the \ourht{} discussed in Section~\ref{sec:unordered} to implement the frontiers with details in Appendix~\ref{sec:bfs-rotating}.
This avoids the writes to check the global array.
We also observed that, once the frontier size fits into the \largemem{}, we do not require any writes to traverse the newly visited vertices.
We show the average and maximum frontier sizes of the graphs on which we experiment in Table~\ref{tab:BFS-stats}.
To the best of our knowledge, there is no graph invariant to capture this property of a graph, and we believe that it can be an interesting topic for further study.
This algorithm is indicated as the \emph{BFS on RA} in Figure~\ref{fig:bfs}, and more details of the implementation are given in the appendix.

The previous algorithm works well on graph with larger diameters, but not on social networks.
We then introduce the bidirectional version on s-t shortest paths, that overcomes the disadvantages the previous algorithm.
More analysis and details of this version are given in Appendix~\ref{sec:bfs-bidir}.

\mysubparagraph{Experiment.}
Our experiment, fully shown in Appendix~\ref{sec:graph}, is based on eight graphs that are synthesized or from SNAP~\cite{leskovec2014snap}.
We show a significant improvement on all eight graphs with various cache sizes, compared to the classic queue-based implementations.
Figure~\ref{fig:bfs} is the bar chart that shows the trends of the four implementations
When $\wcost=10$, we show an up to 8-fold improvement on SSSP, and up to 43-fold improvement on s-t shortest-paths.
For $\wcost=100$, the improvement is more stable, which is 69 on SSSP and 71 on s-t shortest-paths.
Meanwhile, the new algorithm requires less I/O cost in almost all combinations of input instances and cache parameters.

\mysubparagraph{Conclusions.}
We discuss how to efficiently implement BFS in the asymmetric setting and experiment the I/O performance for four implementations on a variety of undirected graphs.
We show that for pairwise distance query, our bidirectional BFS using \rotating{} shows an overwhelming advantage in all cases we tested.
For single-source shorest-paths, the unidirectional BFS using \rotating{} has a better performance if the cache can hold each frontier.

\input{dijk-fig}

\subsection{Dijkstra's Algorithm}

Dijkstra's Algorithm~\cite{dijkstra1959} computes single-source shortest paths on non-negative weighted graphs.
Although Dijkstra's Algorithm is efficient regarding the work (time complexity), the classic heap-based implementation requires $O(\wcost{}m\log (nB/M))$ reads and writes.

For write-efficiency, Blelloch et al.~\cite{blelloch2016efficient} discussed a variant called \emph{Phased Dijkstra}.
This algorithm only requires linear writes, but it is just explained at a high level and without much details.
In this paper, we supplement the pseudocode, data structure design, and implementation details in Appendix~\ref{sec:dijk}.

Based on the implementation, we conduct various experiment to show the asymmetric I/O efficiency.
In Figure~\ref{fig:dijk}, we show the trend of the relative I/O cost of the classic Dijkstra and phased Dijktra with various cache sizes on different graphs.
We show that phased Dijkstra outperforms classic Dijkstra in most cases except for the only case on social networks with very small cache size, and the improvement on I/O cost in all cases is up to 3 and 7.6 when $\wcost$ is 10 and 100.
This result is based on a specific set of parameters of the algorithm and the \static{} cache policy, so we also show results on other cache policies and parameters and the improvement is consistent.

\myparagraph{Conclusions}
We discussed phased Dijkstra and experiment its performance on a variety of graphs.
The high-level idea is to fit the computation within the \smallmem{} (i.e.\ the cache) and thus requires no intermediate writes to the large asymmetry memory.
The experimental results show that phased Dijkstra consistently outperforms the binary-heap version on I/O cost except for the combination of small $\wcost$ ($=10$), small cache size, and on social networks.
Although phased Dijkstra contains some parameters, we also show that they do not affect the efficiency of phased Dijkstra when they are within a reasonable large range.
A similar case also holds for different cache policies.

Notice that the idea here that fits the computation in the \smallmem{} can also be applied to computing minimum spanning tree, sorting, and many other problems. 

==> graph-intro-vldb.tex <==
\section{Dijkstra's Algorithm}

In this paper we discuss two of the most commonly-used graph-traversing algorithms: Breadth-first search (BFS), and Dijkstra's Algorithm.  We show that with appropriate implementations, these algorithms can write much fewer to the main memory, comparing to the classic implementations.

Throughout this section we assume the input graph $G=(V,E)$ contains $n=|V|$ vertices and $m=|E|$ edges.
%graph, frontier.

%\input{BFS}

\input{dijk}


==> hashtable-fig.tex <==
\begin{figure*}[!h!t]
\small
\begin{center}
    \begin{minipage}[t]{0.4\textwidth}
        \includegraphics[width=\textwidth]{figs/ht/hashtable10}\\ \centering{\small (a) $\wcost=10$}
    \end{minipage}~~~
    \begin{minipage}[t]{0.4\textwidth}
        \includegraphics[width=\textwidth]{figs/ht/hashtable100}\\ \centering{\small (b) $\wcost=100$}
    \end{minipage}
\vspace{.5em}
    \captionof{figure}{Relative I/O cost of \ourht{} with different $k$.  The I/O cost is divided by the $k=1$ case. Numbers are from Table~\ref{tab:hashtable-weighted}.}\label{fig:hashtable}
\end{center}
\vspace{-2em}
\end{figure*}


==> hashtable-tab-fig.tex <==
\begin{figure*}[!h!t]
\small
\def\arraystretch{1.2}
  \centering
  $10^6$ insertions, $\alpha\times 10^6$ queries where $\alpha$ is from 0 to 8, cache size is 10,000 cache-lines.
    \begin{tabular}{p{.5cm}<{\centering}|rr|p{.65cm}<{\raggedleft}r|p{.65cm}<{\raggedleft}r|p{.65cm}<{\raggedleft}r|p{.65cm}<{\raggedleft}r|p{.65cm}<{\raggedleft}r|p{.65cm}<{\raggedleft}r|p{.65cm}<{\raggedleft}r}\toprule
    %\multirow{2}[0]{*}{$\bf k$}
     $\bm{\alpha}$& \multicolumn{2}{c|}{\textbf{0}} & \multicolumn{2}{c|}{\textbf{1/8}} & \multicolumn{2}{c|}{\textbf{1/4}} & \multicolumn{2}{c|}{\textbf{1/2}} & \multicolumn{2}{c|}{\textbf{1}} & \multicolumn{2}{c|}{\textbf{2}} & \multicolumn{2}{c|}{\textbf{4}} & \multicolumn{2}{c}{\textbf{8}} \\%\cline{2-17}
     \hline
          & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c|}{\textbf{WT}} & \multicolumn{1}{c}{\textbf{~~RT}} & \multicolumn{1}{c|}{\textbf{WT}} & \multicolumn{1}{c}{\textbf{~~RT}} & \multicolumn{1}{c|}{\textbf{WT}} & \multicolumn{1}{c}{\textbf{~~RT}} & \multicolumn{1}{c|}{\textbf{WT}} & \multicolumn{1}{c}{\textbf{~~RT}} & \multicolumn{1}{c|}{\textbf{WT}} & \multicolumn{1}{c}{\textbf{~~RT}} & \multicolumn{1}{c|}{\textbf{WT}} & \multicolumn{1}{c}{~~RT} & \multicolumn{1}{c|}{\textbf{WT}} & \multicolumn{1}{c}{\textbf{~~RT}} & \multicolumn{1}{c}{\textbf{WT}} \\\hline
    \textbf{k=1}     & 1.35  & 1.17  & 1.44  & 1.18  & 1.52  & 1.19  & 1.69  & 1.21  & 2.02  & 1.24  & 2.68  & 1.27  & 4.00  & 1.31  & 6.64  & 1.34 \\
    \textbf{k=2}     & 0.85  & 0.79  & 1.06  & 0.84  & 1.23  & 0.87  & 1.54  & 0.91  & 2.09  & 0.96  & 3.11  & 1.00  & 5.07  & 1.03  & 8.94  & 1.05 \\
    \textbf{k=3}     & 0.76  & 0.72  & 1.08  & 0.80  & 1.32  & 0.85  & 1.73  & 0.90  & 2.44  & 0.95  & 3.76  & 0.99  & 6.31  & 1.02  & 11.32 & 1.05 \\
    \textbf{k=4}     & 0.70  & 0.67  & 1.11  & 0.78  & 1.40  & 0.82  & 1.89  & 0.88  & 2.74  & 0.93  & 4.30  & 0.97  & 7.33  & 1.00  & 13.31 & 1.03 \\
    \bottomrule
    \end{tabular}%
  \captionof{table}{Numbers of \rwt{s} of \ourht{s} with different query/insert ratios.  Numbers of \rwt{s} are divided by 1M.}
  \label{tbl:hashtable-raw}%
  \medskip
  The I/O costs of \ourht{s} with the same settings in Table~\ref{tbl:hashtable-raw}.
    \begin{tabular}{p{.5cm}<{\centering}|r@{ }@{ }@{ }r@{ }@{ }@{ }r@{ }@{ }@{ }r@{ }@{ }@{ }r@{ }@{ }@{ }r@{ }@{ }@{ }r@{ }@{ }@{ }r|r@{ }@{ }@{ }r@{ }@{ }@{ }r@{ }@{ }@{ }r@{ }@{ }@{ }r@{ }@{ }@{ }r@{ }@{ }@{ }r@{ }@{ }@{ }r}\toprule
     & \multicolumn{8}{c|}{$\bm{\wcost{}=10}$}                                      & \multicolumn{8}{c}{$\bm{\wcost{}=100}$} \\
%\cline{2-17}\multicolumn{1}{c|}{\multirow{2}[0]{*}{\bf k}}
\hline
          $\bm{\alpha}$& \multicolumn{1}{c}{\textbf{0}} & \multicolumn{1}{c}{\textbf{1/8}} & \multicolumn{1}{c}{\textbf{1/4}} & \multicolumn{1}{c}{\textbf{1/2}} & \multicolumn{1}{c}{\textbf{1}} & \multicolumn{1}{c}{\textbf{2}} & \multicolumn{1}{c}{\textbf{4}} & \multicolumn{1}{c|}{\textbf{8}} & \multicolumn{1}{c}{\textbf{0}} & \multicolumn{1}{c}{\textbf{1/8}} & \multicolumn{1}{c}{\textbf{1/4}} & \multicolumn{1}{c}{\textbf{1/2}} & \multicolumn{1}{c}{\textbf{1}} & \multicolumn{1}{c}{\textbf{2}} & \multicolumn{1}{c}{\textbf{4}} & \multicolumn{1}{c}{\textbf{8}} \\
\hline
    \textbf{k=1}     & 13.01 & 13.22 & 13.42 & 13.78 & 14.39 & 15.40 & 17.08 & 20.02 & 117.87 & 119.29 & 120.54 & 122.67 & 125.79 & 129.93 & 134.77 & 140.47 \\
    \textbf{k=2}     & \textcolor[rgb]{ 0,  0,  1}{8.75} & \textcolor[rgb]{ 0,  0,  1}{9.47} & \textcolor[rgb]{ 0,  0,  1}{9.96} & \textcolor[rgb]{ 0,  0,  1}{10.67} & \textcolor[rgb]{ 1,  0,  0}{\underline{11.65}} & \textcolor[rgb]{ 1,  0,  0}{\underline{13.08}} & \textcolor[rgb]{ 1,  0,  0}{\underline{15.38}} & \textcolor[rgb]{ 1,  0,  0}{\underline{19.48}} & \textcolor[rgb]{ 0,  0,  1}{79.87} & \textcolor[rgb]{ 0,  0,  1}{85.14} & \textcolor[rgb]{ 0,  0,  1}{88.45} & \textcolor[rgb]{ 0,  0,  1}{92.78} & \textcolor[rgb]{ 0,  0,  1}{97.71} & \textcolor[rgb]{ 0,  0,  1}{102.89} & \textcolor[rgb]{ 0,  0,  1}{108.18} & \textcolor[rgb]{ 1,  0,  0}{\underline{114.40}} \\
    \textbf{k=3}     & \textcolor[rgb]{ 0,  0,  1}{7.99} & \textcolor[rgb]{ 0,  0,  1}{9.10} & \textcolor[rgb]{ 0,  0,  1}{9.77} & \textcolor[rgb]{ 1,  0,  0}{\underline{10.66}} & \textcolor[rgb]{ 0,  0,  1}{11.90} & \textcolor[rgb]{ 0,  0,  1}{13.65} & \textcolor[rgb]{ 0,  0,  1}{16.54} & 21.81 & \textcolor[rgb]{ 0,  0,  1}{73.06} & \textcolor[rgb]{ 0,  0,  1}{81.35} & \textcolor[rgb]{ 0,  0,  1}{85.84} & \textcolor[rgb]{ 0,  0,  1}{91.27} & \textcolor[rgb]{ 0,  0,  1}{97.01} & \textcolor[rgb]{ 0,  0,  1}{102.65} & \textcolor[rgb]{ 0,  0,  1}{108.65} & \textcolor[rgb]{ 0,  0,  1}{116.28} \\
    \textbf{k=4}     & \textcolor[rgb]{ 1,  0,  0}{\underline{7.41}} & \textcolor[rgb]{ 1,  0,  0}{\underline{8.86}} & \textcolor[rgb]{ 1,  0,  0}{\underline{9.64}} & \textcolor[rgb]{ 0,  0,  1}{10.66} & \textcolor[rgb]{ 0,  0,  1}{12.01} & \textcolor[rgb]{ 0,  0,  1}{14.00} & 17.37 & 23.59 & \textcolor[rgb]{ 1,  0,  0}{\underline{67.85}} & \textcolor[rgb]{ 1,  0,  0}{\underline{78.61}} & \textcolor[rgb]{ 1,  0,  0}{\underline{83.76}} & \textcolor[rgb]{ 1,  0,  0}{\underline{89.60}} & \textcolor[rgb]{ 1,  0,  0}{\underline{95.53}} & \textcolor[rgb]{ 1,  0,  0}{\underline{101.34}} & \textcolor[rgb]{ 1,  0,  0}{\underline{107.69}} & \textcolor[rgb]{ 0,  0,  1}{116.13} \\
    \bottomrule
    \end{tabular}%
  \caption{The I/O costs of \ourht{s} with different query/insert ratios.  The write-read ratio $\wcost{}$ are selected to be typical projected values 10 (latency, bandwidth) and 100 (energy).  Results are based on the numbers in Table~\ref{tbl:hashtable-raw}.  Numbers in red with underlines indicate the best choice of $k$ that minimizes the I/O cost in this setting, and numbers in blue indicate better I/O costs comparing to the classic hash table implementation (i.e.\ $k=1$).}
  \label{tab:hashtable-weighted}%
%\end{table*}
%\begin{figure*}
\begin{center}
    \begin{minipage}[t]{0.4\textwidth}
        \includegraphics[width=\textwidth]{figs/ht/hashtable10}\\ \centering{\small (a) $\wcost=10$}
    \end{minipage}~~~
    \begin{minipage}[t]{0.4\textwidth}
        \includegraphics[width=\textwidth]{figs/ht/hashtable100}\\ \centering{\small (b) $\wcost=100$}
    \end{minipage}
\vspace{.5em}
    \captionof{figure}{Relative I/O cost of \ourht{} with different $k$.  The I/O cost is divided by the $k=1$ case. Numbers are from Table~\ref{tab:hashtable-weighted}.}\label{fig:hashtable}
\end{center}
\vspace{-2em}
\end{figure*}


==> ht-full-exp.tex <==
\section{Full Experiments for \ourht{}}\label{sec:unordered-exp}

\input{hashtable-other-tab}

In the experiment we test the performance of our \ourht{}, including the numbers of \cm{s} and \wrt{s}, I/O costs, and wall-clock running time, on different patterns of queries.
In all experiments, we insert 1 million elements, each of which is a 4-byte integer, into the hash table, and we vary the number of queries.
The simulated cache contains 10,000 cache-lines, and for wall-clock running time we run the code on a PC with Intel i7-2600 CPU and 8GB RAM.
The occupancy rate is set to be $l=0.2$ and $r=0.8$.
We tried other parameters ($r$ between 0.6 and 0.8 and $l=r/4$), and the results are slightly changed but all conclusions drawn in this section remains unchanged.

\myparagraph{Non-deletion case.}
A number of applications, like webpage caching or the breadth-first searches, only insert but never delete elements in a hash table.
Since this is a simpler case, our experiment starts here without considering deletions.
We first show the relationship between $k$ (the number of hash tables) and the numbers of \cm{s} and \wrt{s} for a variety of insertion / query ratio, and the result is shown in Table~\ref{tbl:hashtable-raw}.
We fix the number of insertions to be one million, and query $\alpha$ times after each insertion. We vary $\alpha$ from 0, 1/8 million, ..., to 8 million.
%For example, when the number of queries is 4 million, four queries will come after each insertion.
The ratio of hit is about 50\% (this ratio affects the I/O cost since a successful query can terminate earlier).
The number of hash tables $k$ varies from 1 to 4.
In Table~\ref{tab:hashtable-weighted}, we show the overall I/O costs, which are the weighted sums assuming two typical values of the write-read ratio $\wcost$, 10 and 100.

We first look at the number of \wrt{s}.
When there is no query (i.e., the first column, just inserting 1 million entries), the numbers of writes are consistent with our analysis for insertions in Section \ref{sec:hashtable}.
The only exception here is that cache can hold a constant fraction of the elements, which batches the writes and reduces the number of transfers.
However, the relative trend across different rows (i.e.\ different $k$) remains unchanged.
Namely, the number of writes always decreases as the increase of $k$ regardless of the ratio between queries and updates.
The percentage of writes is reduced by $33\%$, $40\%$ and $43\%$ when $k=2,3,4$ respectively.
This reduction also shows up in the overall I/O cost in Table~\ref{tab:hashtable-weighted}.

More queries clearly cause more reads, and larger $k$ leads to more reads (since these reads flush the cache-lines, the overall number of writes also increases by the increase of the queries).
The optimal I/O cost is affected by $k$, input distribution, and the write-read ratio $\wcost$.
More queries lead to worse performance with larger $k$, and larger $\wcost$ prefers larger $k$.
In Table~\ref{tab:hashtable-weighted} we underline the numbers indicating the best choice of $k$ in that setting.
Picking $k$ to be 2 or 3 is always a good choice when $\wcost=10$, and 3 or 4 when $\wcost=100$.
%

\myparagraph{Wall-clock running time.}
We also measure the actual running time of the previously stated operations on a PC.
In our current platform and hardware, the write-read ratio is close to 1.
Here we show that, the numbers in Table~\ref{tbl:hashtable-raw} almost match the actual running time shown in Table~\ref{tbl:wallclock}, when plugging $\wcost=1$.
Therefore, it is reasonable to believe that, the I/O cost shown in Table~\ref{tab:hashtable-weighted} can reasonably well project the performance for the future memory, when the bandwidth changes asymmetrically (the argument for energy consumptions holds independently with this running time and other architectural issues).
Meanwhile, in the current platform, if the number of insertion is more than the number of queries, using \ourht{} with $k=2$ improves the performance.

As we stated at the beginning of this section, in this experiment setting, our implementation has a much lower I/O cost comparing to separate chaining.  We run the same experiment using the STL unordered set (with the same hash function and other setups), and our hash table is at least 3-4 times faster in all cases.

\myparagraph{Insertion and deletion case.}
We also tested the performance of \ourht{} on deletions.
%The experiment setting is the same as the non-deletion case, and the only difference is now that we first insert 1 million elements, and then remove them all.
We first insert 1 million elements and then remove them all.
After each insertion or deletion, we query $\alpha$ times. The other settings are the same as the non-deletion case.
The results on the numbers of \cm{} and \wrt{} are shown in Table~\ref{tbl:hashtable-delete-raw}, and the overall I/O cost with write-read ratio $\wcost$ to be 10 and 100 are shown in Table~\ref{tab:hashtable-delete-weighted}.

From the results, we get almost the same trend as the non-deletion case.
Comparing with the classic implementation (i.e., $k=1$), the overall number of \wrt{} is reduced by 25\%, 32\% and 36\% when no queries involved, and the improvement is slightly decreased when more queries come in, since more read accesses flush out the cache-lines.
Notice that, the number of \cm{} required by a deletion is more than that for an insertion, since in each deletion we need to allocate the element in the hash table, which requires to look up at most $k$ cache-lines.
Hence comparing to the non-deletion case, slightly smaller values for $k$ are more preferable.
The best choice of $k$ in each case is underlined and shown in Table~\ref{tab:hashtable-delete-weighted}.
For smaller $\wcost{}=10$ (indicate bandwidth and latency) the best $k$ varies based on different query/update ratios, but $k=2$ is always an acceptable choice.
When considering the energy consumption ($\wcost\approx 100$), a larger $k$, like 3 or 4, is more desirable in all cases.

\hide{
\myparagraph{Breadth-first search as an application.}
In the full version of this paper we discussed our implementations on breadth-first searches (BFS) on graph traversing or searching.
Our algorithms computes the single-source shortest paths (SSSP) or s-t shortest-paths on unweighted graphs, which can further apply to graph radii estimation, eccentricity estimation and betweenness centrality, and as a basic building block for other graph algorithms like graph connectivity, reachability, bridges, biconnected components, and strongly connected components.

There are two technical contributions in our new algorithms: one is the new algorithm design that always constrains the size of the temporal memory used in the search to be the (order of the) maximum size of the any frontier (i.e.\ the set of vertices with the same distance to the source node); the other is the new \ourht{} that acts as the underlying data structure to run BFS, which minimizes the number of writes to the main memory.

With the new BFS algorithm, we show a significant improvement on eight real-world graphs (details of these graphs are provided in Section~\ref{sec:dijk-exp}) with various cache sizes, compared to the classic queue-based implementations.
When $\wcost=10$, we show an up to 8-fold improvement on SSSP, and up to 43-fold improvement on s-t shortest-paths.
For $\wcost=100$, the improvement is more stable, which is 69 on SSSP and 71 on s-t shortest-paths.
Meanwhile, the new algorithm requires less I/O cost in almost all combinations of input instances and cache parameters.
}



==> parallel.tex <==
\section{Cost Models for Parallel Algorithms}

\subsection{The Parallel Random-Access Machine (PRAM) Model}

A \defn{parallel random-access machine (PRAM)} is a shared-memory abstract machine. 
As its name indicates, the PRAM is viewed as the parallel analogy to the random-access machine (RAM).
On this model, there are problem-size-dependent number of processors, each can run a basic operation or read and write to a specific memory location with unit cost.
All processors are synchronized, which means that in every time stamp, every processor proceed one unit of work together.
The cost of an algorithm is estimated using two parameters: the overall time to finish, and the product of this time and the number of processors.

Since multiple processors may access to the same memory, there are several assumptions to handle contentions:
(1) the exclusive-read
exclusive-write (EREW) model, which does not allow for concurrent reads or writes; (2)
the concurrent-read exclusive-write (CREW) model, which allows for concurrent reads
but not concurrent writes; (3) the concurrent-read concurrent-write (CRCW) model, which
allows for both concurrent reads and writes. For the CRCW model,
concurrent writes to a shared location results in either an arbitrary write being recorded
(arbitrary CRCW), or the minimum (or maximum) value being recorded (priority CRCW).

\subsection{Programming Model}

The algorithms assume the nested-parallel model (or nested fork-join parallelism), 
in which a fork specifies procedures that can be called in parallel,
and a join specifies a synchronization point among procedures. The fork and join constructs
can be nested.

More formally, nested parallel computations can be defined inductively in terms of
the composition of sequential and parallel components. At the base case, a strand is a
sequential computation. A task is then a sequential composition of strands and parallel
blocks, where a parallel block is a parallel composition of tasks starting with a fork and
ending with a join.
A nested parallel computation can be modeled (a posteriori) as a series-parallel computation
DAG over the operations of the computation: the tasks in a parallel block are
composed in parallel, and the operations within a strand as well as the strands and parallel
blocks of a task are composed in series in the order they are executed. All operations are
assumed to take a state and return a value and a new state (any arguments are part of the
operation). Vertices in the computation DAG are labeled by their associated operation
(including arguments, but not return values or states). An operation (vertex) u precedes
v if there is a directed path from u to v in the DAG. If there is no directed path in either
direction between u and v, then u and v are logically parallel, meaning that they may be
executed in parallel.

==> sort-fig.tex <==
\begin{figure*}
\begin{center}
    \begin{minipage}[t]{0.45\textwidth}
        \includegraphics[width=\textwidth]{../figs/sort/dir10} \centering{\small (a) $\wcost=10$}
    \end{minipage}~~~
    \begin{minipage}[t]{0.45\textwidth}
        \includegraphics[width=\textwidth]{../figs/sort/dir100} \centering{\small (b) $\wcost=100$}
    \end{minipage}
\vspace{-.5em}
    \captionof{figure}{I/O costs of different sorting algorithms on $10^7$ \textbf{doubles} with various read-write asymmetry $\wcost$.  Numbers are from Table~\ref{tbl:sort}.}\label{fig:addingedges}
\end{center}
\begin{center}
    \begin{minipage}[t]{0.45\textwidth}
        \includegraphics[width=\textwidth]{../figs/sort/ind10} \centering{\small (a) $\wcost=10$}
    \end{minipage}~~~
    \begin{minipage}[t]{0.45\textwidth}
        \includegraphics[width=\textwidth]{../figs/sort/ind100} \centering{\small (b) $\wcost=100$}
    \end{minipage}
\vspace{-.5em}
    \captionof{figure}{I/O costs of different sorting algorithms on $2\times 10^6$ \textbf{pointers} with various read-write asymmetry $\wcost$.  Numbers are from Table~\ref{tbl:sort-ind}.}\label{fig:sort-doubles}
\end{center}
%\vspace{-2em}
%\end{figure*}
\end{figure*}



==> sort-imp.tex <==
\section{More Details of the Sorting Algorithms}\label{sec:sort-imp}

\myparagraph{Quicksort.}  Quicksort is the one of the commonly-used sorting algorithms in both sequential and parallel setting.
It picks a random pivot (or the median among several random samples) that partitions the array into three contiguous subsets containing the input values that are less than, equal to, and larger than the pivot respectively, based on a scan-based approach.
Then two recursive calls are made to the less-than and larger-than subsets, until the base case (we set it to be 16 elements) is reach and the algorithm switch to an insertion sort.  In our implementation, the pivot is selected to be the median of three random positions.

We now analyze the I/O cost of quicksort.
Once the subproblem size is no more than $M$, the \smallmem{} size, the subproblem will fit into the cache and no more read and write transfers are required for this subtask thereafter.
The I/O cost $Q$ is thus $O(\wcost{}n/B\cdot \log (n/M))$, where the number of memory transfers to partition the array in the same recursive level add up to $O(n/B)$ and w.h.p.\ the algorithm requires $O(\log (n/M))$ levels to reach the subtask with size no more than $M$.

\myparagraph{Mergesort.}  Mergesort is another textbook sorting algorithm that is stable and easy to parallel.
The implement of mergesort has different versions and here we discuss an I/O-efficient version.
The algorithm partitions the array into two equal-length parts and recursively sort every subproblem individually.
After the computation of both subtasks is finished, a scan-based process merges the two sorted subsequences into the final output.
To implement the algorithm efficiently, we use the \rotating{} so that every element is moved only once in one merge process.
An extra round of data copy is applied if the latest merge leaves the sorted result in the temporal array.

Similarly to quicksort, no further memory transfers are used in subproblems with size no more than $M$.  Therefore the I/O cost $Q$ of mergesort is also $O(\wcost{}n/B\cdot \log (n/M))$.  More specifically, $Q = (1+\wcost{})n/B\cdot \lceil\log_2(n/M) \rceil$ when $\lceil\log_2(n/M) \rceil$ is even, and otherwise there is an extra $(1+\wcost{})n/B$.

\myparagraph{BST sort.}  BST sort treat the input as an ordered set and all elements are maintained in a binary search tree.
Then the in-order traversal of the tree is the sorted output.  The BST can either be balanced, or does not apply any rotation but the elements are inserted in a random order.
Both cases give I/O cost of $O(n\log n+n\wcost{})$ on $n$ input elements.
It is typically used when the input is adaptive: elements can be inserted and removed from the input while the sorted result can be easily accessed at any time.
In this case, some balancing schemes are required if the insertions and deletions are biased.

In our implementation elements are inserted in a random order, which is done in two phases: the first phase generates $n$ uniformly random integers $a_1,\cdots, a_n$ between 1 to $n$ using some hash functions, and inserting the $a_i$-th elements into the tree with \emph{no} rotations (check whether this element is already inserted before the actual insertion); then in the second phase we insert every uninserted element into the tree in the input order.  This guarantees that w.h.p.\ the gap of the elements inserted in the first phase is $O(\log n)$ in the output order.  Hence the tree depth is $O(\log n)$ disregarding any input order, and thus inserting one element requires $O(\log n)$ reads and two random writes (the boolean flag that this node is inserted, and to change the parent's pointer).

\myparagraph{Samplesort.}  Samplesort is a class of sorting algorithms that is based on divide-and-conquer paradigm with multiple pivots and especially commonly-used in the multicore setting.  To minimize the I/O cost and number of memory transfers, in this paper we discuss a cache-aware implementation of samplesort.

Given the cache size $M$ and block size $B$, if the input size is smaller than $M$ then we simply call quicksort.  Otherwise, we pick $M$ random samples from the input, sort the samples, and pick the $B$-th, $2B$-th, ... , $(M-B)$-th samples as the \textbf{pivots}\footnote{\small If $M<n/B$ then we pick $n/B$ samples, and this will happen only once w.h.p.\ in the algorithm.  In practice we replace $M$ to be $M/c'$ for some small constant $c'>1$ to ensure everything that should be in the cache is actually in the cache.} and they form $M/B$ buckets.  Then for each input element, we binary search (an implicit search tree) its associated bucket.  Finally we again samplesort the elements in each bucket individually and recursively.

The algorithm partition the input into $M/B$ almost equal-size subproblems with $O(n/B)$ read and write transfers.  The I/O cost of this algorithm on average is $\displaystyle O\left({\wcost{}n\over B}\log_{M\over B}{n\over B}\right)$.

The number of \wrt{} of samplesort in our implementation is highly optimized so that one round samplesort only requires three sequential reads and one sequential write per input element.
After picking the pivots, we first loop over the input to binary search the associate bucket of each element.
However, we do not store this value; instead, we only modify the counters of each bucket.
After that, we have known the number of elements in each bucket, and we apply a prefix sum compute the offset of each element.
Finally all elements are distributed to their associated buckets based on the offsets.
The algorithm only requires three reads and one write for each element, and all other operations are all within the cache.
Notice that after one round, the data are stored in another array, so the final results will be moved back to the original array if they happen to be in the other one.



==> sort-table.tex <==
\begin{figure*}[!t]
%\begin{table*}
\centering
\def\arraystretch{1.2}
\small
\begin{tabular}{c|rrr|rrr|rrr|rrr}
\toprule
     \textbf{Cache} &      \multicolumn{ 3}{c|}{\textbf{Quicksort}} &      \multicolumn{3}{c|}{\textbf{Mergesort}} &        \multicolumn{ 3}{c|}{\textbf{BST sort}} &     \multicolumn{3}{c}{\textbf{Samplesort}} \\
     \cline{2-13}

      \textbf{Size} &         \textbf{RT} &         \textbf{WT} &      \textbf{\#comp} &         \textbf{RT} &         \textbf{WT} &      \textbf{\#comp} &         \textbf{RT} &         \textbf{WT} &      \textbf{\#comp} &         \textbf{RT} &         \textbf{WT} &      \textbf{\#comp} \\
\hline
       \textbf{100} &       2.06 &       2.04 &      39.49 &       4.01 &       2.00 &      24.11 &      24.49 &       2.04 &      43.76 &       1.60 &       0.82 &      63.05 \\

      \textbf{1000} &       1.58 &       1.57 &      39.49 &       3.11 &       1.56 &      24.11 &      19.39 &       2.04 &      43.76 &       1.01 &       0.51 &      56.63 \\

     \textbf{10000} &       1.11 &       1.10 &      39.49 &       2.25 &       1.13 &      24.11 &      14.17 &       2.03 &      43.76 &       0.50 &       0.25 &      52.47 \\
\bottomrule
\end{tabular}%\vspace{-1em}
\captionof{table}{Performance of different sorting algorithms on $10^7$ random i.i.d.\ double-precision float-point numbers.  Values in the table are numbers of read and write transfers and comparisons per input element.  Cache size is measured by the number of 64-byte cache-lines.}
\label{tbl:sort}
%\vspace{.5em}
\begin{tabular}{c|rrr|rrr|rrr|rrr}
\toprule
     \textbf{Cache} &      \multicolumn{ 3}{c|}{\textbf{Quicksort}} &      \multicolumn{3}{c|}{\textbf{Mergesort}} &        \multicolumn{ 3}{c|}{\textbf{BST sort}} &     \multicolumn{3}{c}{\textbf{Samplesort}} \\
     \cline{2-13}

      \textbf{Size} &         \textbf{RT} &         \textbf{WT} &      \textbf{\#comp} &         \textbf{RT} &         \textbf{WT} &      \textbf{\#comp} &         \textbf{RT} &         \textbf{WT} &      \textbf{\#comp} &         \textbf{RT} &         \textbf{WT} &      \textbf{\#comp} \\
\hline
       \textbf{100} &      19.83 &       1.14 &      37.68 &      17.04 &       1.02 &      23.30 &      46.24 &       1.93 &      40.93 &       6.19 &       0.79 &      35.97 \\

      \textbf{1000} &      15.57 &       0.91 &      37.68 &      13.42 &       0.81 &      23.30 &      35.30 &       1.92 &      40.93 &       3.93 &       0.45 &      34.34 \\

     \textbf{10000} &      11.12 &       0.67 &      37.68 &       8.96 &       0.56 &      23.30 &      24.65 &       1.90 &      40.93 &       2.38 &       0.38 &      34.43 \\
\bottomrule
\end{tabular}%\vspace{-1em}
\caption{Performance of different sorting algorithms on $2\times10^6$ indices pointing to structures with average size of 64 bytes.  Other setup is the same as that in Table~\ref{tbl:sort}.}
\label{tbl:sort-ind}
%\vspace{-2em}
\end{figure*} 

==> table-dijk-other-dc.tex <==
\begin{figure*}[htbp]
\begin{minipage}[t]{0.41\textwidth}
  \centering
  \small
  \def\arraystretch{1.2}
    \begin{tabular}{l|rr|rr}
    \toprule
    \multicolumn{1}{c|}{\textbf{Cache Policy}} & \multicolumn{2}{c|}{\textbf\splitpool{}} & \multicolumn{2}{c}{\textbf{\static{}}} \\
\cline{1-5}          & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c|}{\textbf{WT}} & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c}{\textbf{WT}} \\
    \hline
    \textbf{2D Grid} & 3.74  & 1.11  & 3.62  & 1.11 \\
    \textbf{3D Grid} & 27.43 & 1.12  & 28.16 & 1.12 \\
    \textbf{PA Roadmap} & 1.84  & 0.88  & 1.89  & 0.52 \\
    \textbf{TX Roadmap} & 1.83  & 0.87  & 1.88  & 0.53 \\
    \textbf{Stan Webgraph} & 81.40 & 1.02  & 81.02 & 1.02 \\
    \textbf{NDU Webgraph} & 21.96 & 1.07  & 22.57 & 1.01 \\
    \textbf{DBLP Network} & 65.20 & 1.11  & 64.75 & 1.10 \\
    \textbf{Youtube Network} & 163.38 & 1.12  & 161.36 & 1.11 \\
\bottomrule
    \end{tabular}%
  \captionof{table}{\label{tbl:dijk-policy}
  Number of \rwt{} of phased Dijkstra on two different cache policies: the \splitpool{} policy and the \static{} policy.  The cache contains 10,000 cache-lines.
  Different policies give very similar performance except for the writes on roadmaps. }
\end{minipage}
\quad
\begin{minipage}[t]{0.55\textwidth}
  \centering
  \small
  \def\arraystretch{1.2}
    \begin{tabular}{@{ }l@{ }|r@{ }r@{ }@{ }r@{ }r@{ }@{ }r@{ }r@{ }@{ }r@{ }r@{ }}
    \toprule
   \multicolumn{1}{@{}c@{ }|}{\textbf{Priority Queue Size}}       & \multicolumn{2}{c}{\textbf{30\%}} & \multicolumn{2}{c}{\textbf{40\%}} & \multicolumn{2}{c}{\textbf{50\%}} & \multicolumn{2}{c}{\textbf{60\%}} \\
\cline{1-9}          & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c}{\textbf{WT}} & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c}{\textbf{WT}} & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c}{\textbf{WT}} & \multicolumn{1}{c}{\textbf{RT}} & \multicolumn{1}{c}{\textbf{WT}} \\
    \hline
    \textbf{2D Grid} & 8.4   & 1.10  & 8.6   & 1.11  & 8.9   & 1.11  & 9.3   & 1.11 \\
    \textbf{3D Grid} & 33.7  & 1.12  & 28.9  & 1.12  & 25.6  & 1.12  & 23.3  & 1.12 \\
    \textbf{PA Roadmap} & 2.7   & 0.48  & 2.8   & 0.52  & 3.0   & 0.58  & 3.2   & 0.66 \\
    \textbf{TX Roadmap} & 2.6   & 0.48  & 2.7   & 0.53  & 2.9   & 0.59  & 3.1   & 0.66 \\
    \textbf{Stan Webgraph} & 94.4  & 1.02  & 82.9  & 1.02  & 72.1  & 1.02  & 67.1  & 1.02 \\
    \textbf{NDU Webgraph} & 26.1  & 1.01  & 22.8  & 1.01  & 20.2  & 1.03  & 18.5  & 1.04 \\
    \textbf{DBLP Network} & 75.1  & 1.10  & 64.9  & 1.10  & 57.3  & 1.10  & 51.5  & 1.11 \\
    \textbf{Youtube Network} & 183.8 & 1.11  & 161.5 & 1.11  & 144.4 & 1.12  & 134.9 & 1.12 \\
    \bottomrule
    \end{tabular}%
  \captionof{table}{\label{tab:dijk-perc}Number of read and write transfers of phased Dijkstra on different priority queue's size.  The overall percentage of priority queue and vertex map varies from 30\% to 60\% comparing to the cache size, which is 10,000 cache-lines.}
\end{minipage}
\end{figure*}% 
